Conditional Invertible Neural Networks for Diverse Image-to-Image Translation

We introduce a new architecture called a conditional invertible neural network (cINN), and use it to address the task of diverse image-to-image translation for natural images. This is not easily possible with existing INN models due to some fundamental limitations. The cINN combines the purely generative INN model with an unconstrained feed-forward network, which efficiently preprocesses the conditioning image into maximally informative features. All parameters of a cINN are jointly optimized with a stable, maximum likelihood-based training procedure. Even though INN-based models have received far less attention in the literature than GANs, they have been shown to have some remarkable properties absent in GANs, e.g. apparent immunity to mode collapse. We find that our cINNs leverage these properties for image-to-image translation, demonstrated on day to night translation and image colorization. Furthermore, we take advantage of our bidirectional cINN architecture to explore and manipulate emergent properties of the latent space, such as changing the image style in an intuitive way.

==> 01_introduction_OLD.tex <==
Diverse image-to-image translation is a particular conditional generation task:
given a conditioning image $Y$, the task is to model the conditional probability distribution $p(X|Y)$
over some images $X$ in a different domain.
`\emph{Diverse}' implies that the model should generate many different $X$ from the distribution, not just a single answer.
More specifically, we only consider the case of paired training data, meaning matching pairs $(x_i, y_i)$ are given in the training set.
Unpaired image-to-image translation is in theory ill-posed, and only possible through inductive bias or explicit regularization.


Generative adversarial networks (GANs) produce ever larger and more realistic samples \cite{karras2017progressive,brock2018large}. Hence they have become the primary choice for a majority of image generation tasks.
As such, their conditional variants (cGANs) would appear to be the natural tool for conditional image generation as well, and they have successfully been applied in many scenarios \cite{ledig2017photo,miyato2018cgans}.
% Conditional generative adversarial networks (cGANs) are the current state-of-the-art for conditional generation,
% being able to generate highly realistic images at large resolutions \cite{karras2017progressive, brock2018large}.
% 
%Despite numerous improvements, significant expertise and computational resources are required
%to find a training configuration for large GANs that is stable, and produces diverse images.
However, a lack in diversity is especially common when the condition itself is an image, and special precautions have to be taken to avoid complete mode collapse 
\cite{}
and training stability continues to pose a challenge.

%More fundamentally, it is difficult to encourage true diversity in a GAN when the discriminator never sees more than one batch of samples at a time.
%High-dimensional domains and strong conditioning signals, like images, only exacerbate this effect.
%TODO: correct this
% However, they suffer from stability issues, and the generated images often lack diversity for a given conditioning, especially if the conditioning itself is an image.

Conditional variational autoencoders (cVAEs) do not suffer from the same problems.
Training is generally stable,
and since every data point is assigned a region in latent space, sampling yields the full variety of data seen during training.
% On the other hand, conditional variational autoencoders (cVAEs) enable conditional generation by learning a latent code, 
% which can be sampled and decoded for conditional generation.
% While their training process is more stable than that of cGANs, they suffer from other problems:
However cVAEs come with drawbacks of their own:
The assumption of a Gaussian posterior on the decoder side implies an L2 reconstruction loss, which is known to cause blurriness. %TODO_LA
In addition, the partition of the latent space into diagonal Gaussians leads to either mode-mixing issues or regions of poor sample quality \cite{kingma2016improved}.
There has also been some success in combining aspects of both approaches for certain tasks, such as \cite{isola2017image,zhu2017toward,park2019semantic}.

\begin{wrapfigure}{R}{0.5\linewidth}
    %\centering
    \includegraphics[width=\linewidth]{figures/bird_quiz.jpg}\vspace{-2mm}
	\caption{Diverse colorizations, which our network created for the same grayscale image. 
    One of them shows ground truth colors, but which?
    Solution at the bottom of next page.
% 	Which is the original color image? Solution will be added to the camera-ready version.
	}%
	\vspace{-10mm}
	\label{fig:BIRD}
\end{wrapfigure}

%Recent auto-regressive models for image generation achieve very promising results \cite{van2016conditional}, but their sequential nature makes them inefficient for higher-dimensional data.

We propose a third approach, by extending Invertible Neural Networks (INNs, \cite{dinh2016density,kingma2018glow,ardizzone2018analyzing}) for the task of {\em conditional} image generation, by adding conditioning inputs to their core building blocks.
INNs are neural networks which are by construction bijective, efficiently invertible, and have a tractable Jacobian determinant.
They represent transport maps between the input distribution $p(\x)$ and a prescribed, easy-to-sample-from latent distribution $p(\z)$.
During training, the likelihood of training samples from $p(\x)$ is maximized in latent space,
while at inference time, $\z$-samples can trivially be transformed back to the data domain.
Previously, INNs have been used successfully for unconditional image generation, e.g.~by \cite{dinh2016density} and \cite{kingma2018glow}. %TODO_LA trivially?

Unconditional INN training is related to that of VAEs, but it compensates for some key disadvantages:
Firstly, since reconstructions are perfect by design, no reconstruction loss is needed, and generated images do not become blurry.
Secondly, each $\x$ maps to exactly one $\z$ in latent space, and there is no need for posteriors $p(\z\,|\,\x)$.
This avoids the VAE problem of disjoint or overlapping regions in latent space.
In terms of training stability and sample diversity, INNs show the same strengths as autoencoder architectures, but with superior image quality.
We find that these positive aspects apply to conditional INNs (cINNs) as well.

One limitation of INNs is that their design restricts the use of some standard components of neural networks, such as pooling and batch normalization layers.
%One drawback of INNs are the architectural constraints which allow invertibility, but preclude some standard building blocks of neural networks like spatial pooling and BatchNorm.
Our conditional architecture alleviates this problem, as the conditional inputs can be preprocessed by a 
{\it conditioning network} with a standard feed-forward architecture, which can be learned jointly with the cINN
to greatly improve its generative capabilities.
%an unconstrained, possibly pretrained feed-forward network that takes over much of the representational burden.
% So far, INNs have not been used to perform conditional image generation.
% If at all, weak conditioning can be performed after training by analyzing the latent space in some way.
% We therefore demonstrate how INNs can be used for conditional generation, as cINNs.
% This is done by conditioning the entire invertible transformation represented by the INN on some additional variables $c$.
We demonstrate the quality of cINNs for conditional image generation and uncover emergent properties of the latent space, for the tasks of conditional MNIST generation and diverse colorization of ImageNet. 

{Given this, we believe that the cINN architecture brings the research field of INNs and other normalizing flow models a substantial step forward. Despite the fact that INNs have received very little attention in the literature in contrast to GANs, we find that cINNs can achieve comparable quality to cGANs, with some remarkable properties absent in cGANs.}
{This includes diverse outputs by default, compared to sparse support or mode collapse in cGANs, 
easier explainability and interpretability of the learned latent representation,
as well as simple and intuitive manipulation and interpolation of generated or existing images.}

\begin{figure}
    %\input{figures/schematic_overview}
    \parbox{0.64\linewidth}{
        \resizebox{\linewidth}{!}{\hspace{-40mm} \input{figures/schematic_overview}}
    } \hfill
    \parbox{0.35\linewidth}{
        \captionof{figure}{
        Illustration of the cINN. It consists of a feed-forward conditioning network (\emph{left half}), and an invertible part (\emph{right half}). \\
        \textbf{\textcolor{Plum}{Purple arrows:}} connections always in the same direction. \\
        \textbf{\textcolor{Orange}{Orange arrows:}} bidirectional connections, depending on training/testing.  \\
        \textbf{\textcolor{Emerald}{Green boxes:}} extracted feature maps $c^{(k)}$. \\
        \textbf{\textcolor{VioletRed}{Pink blocks:}} conditional coupling blocks (CCBs). 
        }
        \label{fig:overview}
    }
\end{figure}



Our work makes the following contributions:
\begin{itemize}
    \item We propose a new architecture called conditional invertible neural network (cINN), which combines an INN with an unconstrained feed-forward network for conditioning. 
    It generates diverse images with high realism on par with existing approaces, while adding some noteworthy and useful properties.

    \item We demonstrate a stable, maximum likelihood-based training procedure for jointly optimizing the parameters of the INN and the conditioning network.  
    We show that our training causes the conditioning network to extract the most informative features from the condition, measured by the mutual information.
    
    \item We take advantage of our bidirectional cINN architecture to explore and manipulate emergent properties of the latent space. We illustrate this for MNIST digit generation and image colorization. 

    %OLD \item We are the first to implement conditional image generation with an INN, producing sharp images without the drawbacks of cGANs.
    %\item We reduce the architectural limitations of INNs by including unconstrained feed-forward networks in our architecture.
    %\item By construction, our model does not experience mode collapse and generates highly diverse, sharp samples.
    %\item We are able to take advantage of the bidirectional model to explore and manipulate emergent properties of the latent space.
\end{itemize}
\vspace{-10mm}


==> 02_related_work_OLD.tex <==
\noindent
\ttodo{also compare to winkler, waveglow, ib-inn, for con. genenration (-> no conditioning network)}
%{\bf Conditional Generative Modeling.} 
Modern generative models learn to transform noise (usually sampled from multivariate Gaussians) into desired target distributions.
Methods differ by the model-family these transformations are picked from and by the losses determining optimal solutions.

Conditional generative adversarial networks (cGANs, \cite{mirza2014conditional}) train a pair of neural networks: %a {\em generator} transforming condition-and-noise-pairs to images, and a {\em discriminator}, which penalizes when generated images look unrealistic. 
a {\em generator} transforms a pair of conditioning and noise vectors to images, and a {\em discriminator} penalizes unrealistic looking images.
The conditioning information is either concatenated to the noise \cite{mirza2014conditional}, or fed into the network via conditional batch-norm layers \cite{dumoulin2017learned,huang2017arbitrary,park2019semantic}. 
Ensuring diversity of the generated images (for fixed conditioning) appears to be challenging in this approach. 
Recent BigGANs \cite{brock2018large} successfully address this problem by using very large networks and batch sizes, but require parallel training on up to 512 TPUs.
PacGANs \cite{lin2018pacgan} employ augmented discriminators, which evaluate entire batches of real or generated images together rather than one image at a time.
CausalGANs \cite{kocaoglu2017causalgan} train two additional discriminator networks, called ``labeler'' and ``anti-labeler'', with the latter explicitly penalizing the lack of diversity.
Pix2pix \cite{isola2017image} addresses the important special case when the target is conditioned on an image in a different modality, e.g.~to generate satellite images from maps. 
In addition to the discriminator loss, it minimizes the L1 distance between  generated and ground-truth targets using a paired training set, which contains corresponding images from both modalities.
This leads to impressive image quality, but lack of diversity seems to be an especially hard problem in this case. 
In contrast, our method does not need explicit precautions to promote diversity.
%\CR{here a sentences needed to say: in contrast to GAN we dont have mode colalps or betetr diversity. or say all GAN}

Bidirectional architectures augment generator networks with complementary encoder networks that learn the generator's inverse and enable reconstruction losses, which exploit cycle consistency requirements.
Conditional variational autoencoders (cVAEs, \cite{sohn2015cvae}) replace all distributions in a standard VAE \cite{kingma2013auto} by the appropriate conditional distributions, and are trained to minimize the evidence lower bound (ELBO loss).
Since variational distributions are typically Gaussian, the reconstruction penalty is equivalent to squared loss, resulting in rather blurry generated images.
This is avoided by AGE networks \cite{ulyanov2018it} and CycleGANs \cite{zhu2017cyclegan}, which combine standard cGAN discriminators with L1 reconstruction loss in the data domain, 
and bidirectional conditional GANs \cite{jaiswal2017bidirectional}, which extend the GAN discriminator to act on the distributions in data and latent space jointly.
SPADE \cite{park2019semantic}, building upon pix2pix and pix2pixHD \cite{wang2018high}, augments cGANs with additional VAE encoders to shape the latent space such that diversity is ensured.  

Instead of enforcing bijectivity through cycle losses,
invertible neural networks are bidirectional by design, since encoder and generator are realized by forward and backward processing within a single bijective model. 
We focus on architectures whose forward and backward pass require the same computational effort.
The coupling layer designs pioneered by NICE \cite{dinh2014nice} and RealNVP \cite{dinh2016density} emerged as very powerful and flexible model families under this restriction.
Using additive coupling layers, i-RevNets \cite{jacobsen2018irevnet} demonstrated that the lack of information reduction from data space to latent space does not cause overfitting.
The Glow architecture \cite{kingma2018glow} combines affine coupling layers with invertible 1x1 convolutions and achieves impressive attribute manipulations (e.g. age, hair color) in generated faces images.
This approach was recently generalized to video by \cite{kumar2019videoflow}.

Thanks to tractable Jacobian determinants, the coupling layer architecture enables maximum likelihood training \cite{dinh2014nice,dinh2016density}, but experimental comparisons with other training methods are inconclusive so far.
For instance, \cite{danihelka2017comparison} found minimization of an adversarial loss to be superior to maximum likelihood training in RealNVPs, 
\cite{schirrmeister2018generative} trained i-RevNets in the same manner as adversarial auto-encoders, i.e.~with a discriminator acting in latent rather than data space,
and Flow-GANs \cite{grover2018flow} performed best using bidirectional training, a combination of maximum likelihood and adversarial loss.
On the other hand, maximum likelihood training worked well within Glow \cite{kingma2018glow}, and i-ResNets \cite{behrmann2018invertible} could even be trained with approximated Jacobian determinants.
In this work we reinforce the view that high-quality generative models can be trained by maximum likelihood loss alone.
To the best of our knowledge, we are the first to apply the coupling layer design for {\em conditional} generative models, 
with the exception of \cite{ardizzone2018analyzing}, who use it to compute posteriors for (relatively small) inverse problems, but do not consider image generation.

{\bf Colorization.}
State-of-the-art regression models for colorization produce visually near-perfect images \cite{iizuka2016let,zhang2016colorful,larsson2016learning}, 
but do not account for the ambiguity inherent in this inverse problem.
To address this, models would ideally define a conditional distribution of plausible color images for a given grayscale input, instead of just returning a single ``best'' solution.

%Popular existing approaches for diverse colorization predict per-pixel color histograms from a U-Net \cite{zhang2016colorful} or from hypercolumns of an adapted VGG network \cite{larsson2016learning}.
%However, sampling from these local histograms independently can not lead to a spatially consistent colorization,
%requiring additional heuristic post-processing steps to avoid artefacts.

%--------------------------------- Version 1:
%
In terms of generative models, both VAEs \cite{deshpande2017learning}, cGANs \cite{isola2017image,cao2017unsupervised} have been proposed for the task. 
However, their solutions do not reach the quality of the regression-based models, and cGANs in particular often lack diversity.
Auto-regressive models \cite{guadarrama2017pixcolor} and CRFs \cite{royer2017probabilistic} have also been applied,
but are computationally very expensive and unable to scale to realistic image sizes..
%To compensate, modifications and extensions to generative approaches have been developed, 
%such as auto-regressive models \cite{guadarrama2017pixcolor} and CRFs \cite{royer2017probabilistic}.
%However, these methods are computationally very expensive and often unable to scale to realistic image sizes.

Conceptually closest to our proposed method is the work of \cite{ulyanov2018it}, 
where an encoder network maps color information to a latent space and a generator network learns the inverse transform conditioned on the grayscale image.
Their experiments however are limited to a data set with only cars, and just three latent dimensions, leading to global, but no local diversity.

%--------------------------------- Version 2:
%
%Building on an alternative method based on an autoencoder with multi-modal latent distribution \cite{deshpande2017learning}, which allows to capture diverse color field embeddings, \cite{messaoud2018structural} employ a fully connected Gaussian CRF to model pixel dependencies.
%This ensures global consistency in the sampled colorizations, but inference in the random field comes at a high computational cost.
%Recently proposed sequential auto-regressive models based on Pixel-CNN \cite{guadarrama2017pixcolor, royer2017probabilistic} offer an even higher trade-off between sample quality and inference time -- to an extent where their application on realistic image sizes becomes infeasible.
%While generative-adversarial networks have been investigated for diverse colorization, generating a true variety of color images remains challenging even on restricted data sets \cite{cao2017unsupervised}.
%Conceptually closest to our proposed method is the work of \cite{ulyanov2018it}, where an encoder network maps color information to a latent space and a generator network learns the inverse transform, both conditioned on the gray-scale image.
%Their experiments however are limited to a data set with only cars, and just three latent dimensions.
%
%---------------------------------
%
In contrast to the above, our flow-based cINN generates diverse colorizations in one standard feed-forward pass. It 
models the distribution of all pixels jointly, and allows for meaningful latent space manipulations.

==> figs_map2sat/pca_features.tex <==
\resizebox{\textwidth}{!}{
    \includegraphics[width=3cm, trim=0 1.8cm 1.0cm 0, clip]{figs_map2sat/009_y.png} %
    \includegraphics[width=3cm, trim=0 1.8cm 1.0cm 0, clip]{figs_map2sat/009_01_003.png} %
}\\
\resizebox{\textwidth}{!}{
    \includegraphics[width=3cm, trim=0 1.8cm 1.0cm 0, clip]{figs_map2sat/009_02_006.png} %
    \includegraphics[width=3cm, trim=0 1.8cm 1.0cm 0, clip]{figs_map2sat/009_03_003.png} %
}
